Enhancing Computer Programming Education with LLMs: A Study on Effective Prompt Engineering for Python Code Generation

Large language models (LLMs) and prompt engineering hold significant potential for advancing computer programming education through personalized instruction. This paper explores this potential by investigating three critical research questions: the systematic categorization of prompt engineering strategies tailored to diverse educational needs, the empowerment of LLMs to solve complex problems beyond their inherent capabilities, and the establishment of a robust framework for evaluating and implementing these strategies. Our methodology involves categorizing programming questions based on educational requirements, applying various prompt engineering strategies, and assessing the effectiveness of LLM-generated responses. Experiments with GPT-4, GPT-4o, Llama3-8b, and Mixtral-8x7b models on datasets such as LeetCode and USACO reveal that GPT-4o consistently outperforms others, particularly with the "multi-step" prompt strategy. The results show that tailored prompt strategies significantly enhance LLM performance, with specific strategies recommended for foundational learning, competition preparation, and advanced problem-solving. This study underscores the crucial role of prompt engineering in maximizing the educational benefits of LLMs. By systematically categorizing and testing these strategies, we provide a comprehensive framework for both educators and students to optimize LLM-based learning experiences. Future research should focus on refining these strategies and addressing current LLM limitations to further enhance educational outcomes in computer programming instruction.

==> sections/notes.tex <==
Title:  How to generate the best Python code for School Problem


Introduction

	Motivation 

		Value for Education – 1) testing the limit of LLM; 2) help the students

Problem:

	Using LLM to generate the code with good quality 
	What is good quality – model to evaluate (third-party) 

	


Related Work 

	Paper 
	Generation Discussion of Using LLM
		Focus on education 

	Generate Code 

Architecture:
	Missing 

Solution:
	Transfer Learning (comparison without any prior knowledge zero shot)
	
	Problem Group:
		Algorithm
			Speed
			Memory 
			Accuracy 

Extract a good example.
	Good in which aspect 
		Encapsulation 
		Not leakage of information (secure) 
		No memory leaking. 
		Less memory usage 
		Fast 

Request (single category learning) 

	Transfer learning:

1.	Class Encapsulation   Judge 
2.	No memory leakage  Judge 

Two-category Learning (Class + no memory leakage) 

	Two categories   Judge 

Multiple category learning 
	Judge 


Zero, One, two, multiple 

Discussion:
	Chart and example (choose some questions)

	Compared with human results. 
Conclusion 

